On a stochastic differential equation arising in a price impact model

We provide sufficient conditions for the existence and uniqueness of solutions to a stochastic differential equation which arises in a price impact model. These conditions are stated as smoothness and boundedness requirements on utility functions or Malliavin differentiability of payoffs and endowments.

==> style.tex <==
% Packages

\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
%\usepackage[dvips]{color}
%\usepackage{epsfig}
%\usepackage{graphicx}
%% \usepackage{harvard}
 \usepackage{mathrsfs}
\usepackage[numbers]{natbib}
\usepackage[colorinlistoftodos, textwidth=4cm, shadow]{todonotes}

\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary}%
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}%
\newtheorem{Definition}[Theorem]{Definition}%
\newtheorem{Example}[Theorem]{Example} %
\newtheorem{Question}[Theorem]{Question}%
\newtheorem*{Acknowledgments}{Acknowledgments} %

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %


% Useful commands

\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\braces}[1]{\left\lbrace{#1}\right\rbrace}
\newcommand{\descr}[2]{\left\lbrace{#1}:\; #2 \right\rbrace}
\newcommand{\dhvec}[2]{\begin{pmatrix}
  #1 & #2
\end{pmatrix}
}
\newcommand{\dvec}[2]{\begin{pmatrix}
   #1 \\
  #2
\end{pmatrix}
}
\newcommand{\idvec}{\mathbf{1}}
\newcommand{\seq}[1]{$\left(#1^n\right)_{n\geq 1}$}
\newcommand{\set}{\triangleq}
\newcommand{\ip}[2]{\left\langle
    #1,#2 \right\rangle}
\newcommand{\ind}[1]{1_{\braces{#1}}}
\newcommand{\setind}[1]{1_{#1}}
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\mtext}[1]{\;\text{#1}\;} % text in the middle of a formula
\newcommand{\norm}[1]{\lVert#1\rVert} %
\newcommand{\transpose}[1]{{#1}^T}
\newcommand{\itemFref}[1]{{\rm (F\ref{#1})}}
\newcommand{\itemGref}[1]{{\rm (G\ref{#1})}}
\newcommand{\Cov}[3]{\cov_{#1}[#2,#3]}
\newcommand{\Var}[2]{\var_{#1}[#2]}

% Mathematical operators

\DeclareMathOperator*{\argmax}{arg\:max}
\DeclareMathOperator*{\argmin}{arg\:min}
\DeclareMathOperator{\boundary}{\partial}
\DeclareMathOperator*{\closure}{cl}
\DeclareMathOperator{\cov}{Cov}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator*{\interior}{int}
\DeclareMathOperator*{\ri}{ri}
\DeclareMathOperator*{\rank}{rank}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\var}{Var}
\DeclareMathOperator{\const}{const}

% Environments

\newcommand{\envspace}{\vspace{2mm}}
\newenvironment{ToDo}{\envspace
  \noindent {\textbf{Things to do:}}  \sf}{\envspace }

%%%%%%%%%%%%%%%%%%% Peter's additions

\renewcommand{\mathcal}{\mathscr}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\fA}{\mathfrak{A}}
\newcommand{\fB}{\mathfrak{B}}
\newcommand{\fC}{\mathfrak{C}}
\newcommand{\fD}{\mathfrak{D}}
\newcommand{\fE}{\mathfrak{E}}
\newcommand{\fF}{\mathfrak{F}}
\newcommand{\fG}{\mathfrak{G}}
\newcommand{\fH}{\mathfrak{H}}
\newcommand{\fI}{\mathfrak{I}}
\newcommand{\fJ}{\mathfrak{J}}
\newcommand{\fK}{\mathfrak{K}}
\newcommand{\fL}{\mathfrak{L}}
\newcommand{\fM}{\mathfrak{M}}
\newcommand{\fN}{\mathfrak{N}}
\newcommand{\fO}{\mathfrak{O}}
\newcommand{\fP}{\mathfrak{P}}
\newcommand{\fQ}{\mathfrak{Q}}
\newcommand{\fR}{\mathfrak{R}}
\newcommand{\fS}{\mathfrak{S}}
\newcommand{\fT}{\mathfrak{T}}
\newcommand{\fU}{\mathfrak{U}}
\newcommand{\fV}{\mathfrak{V}}
\newcommand{\fW}{\mathfrak{W}}
\newcommand{\fX}{\mathfrak{X}}
\newcommand{\fY}{\mathfrak{Y}}
\newcommand{\fZ}{\mathfrak{Z}}

\newcommand{\dAA}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\bRR}{\overline{\mathbb{R}}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

\renewcommand{\epsilon}{\varepsilon}

\newcommand{\supp}{\operatorname{\mathrm{supp}}}
\newcommand{\esssup}{\operatorname*{\mathrm{ess\,sup}}}
\newcommand{\essinf}{\operatorname*{\mathrm{ess\,inf}}}
\newcommand{\essinfext}[1][\P]{#1\text{\rm--}\essinf}
\newcommand{\esssupext}[1][\P]{#1\text{\rm--}\esssup}
\newcommand{\condessinf}[2][\cF_t]{\essinfext[#1]#2}
\newcommand{\condesssup}[2][\cF_t]{\esssupext[#1]#2}
\newcommand{\Dom}{\operatorname{\mathrm{Dom}}}
\newcommand{\myexp}[1]{\exp\left(#1\right)}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
\newcommand{\br}[1]{\left\langle #1 \right\rangle}
\newcommand{\rbr}[1]{\left( #1 \right)}
\newcommand{\cbr}[1]{\left[ #1 \right]}
\newcommand{\sumno}{\sum\nolimits}

\renewcommand{\P}{\PP}
\newcommand{\Pas}{\text{$\P$--a.s.}}
\newcommand{\E}{\EE}
\newcommand{\Prob}[2][]{\P^{#1}\left[#2\right]}
\newcommand{\ttext}[1]{\quad \text{#1} \quad}

